EDA: Easy Data Augmentation Techniques for Boosting Performance on Text Classification Tasks

We present EDA: easy data augmentation techniques for boosting performance on text classification tasks. EDA consists of four simple but powerful operations: synonym replacement, random insertion, random swap, and random deletion. On five text classification tasks, we show that EDA improves performance for both convolutional and recurrent neural networks. EDA demonstrates particularly strong results for smaller datasets; on average, across five datasets, training with EDA while using only 50% of the available training set achieved the same accuracy as normal training with all available data. We also performed extensive ablation studies and suggest parameters for practical use.

==> figures/single_saturation.tex <==

\pgfplotsset{width=6cm,compat=1.9}
\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
\begin{centering}
\begin{tikzpicture}
\begin{axis}[
    %title={Performance on Five Datasets},
    xlabel={Percent of Dataset (\%)},
    ylabel={Average Accuracy},
    xmin=0, xmax=100,
    ymin=0.6, ymax=1,
    xtick={0,20,40,60,80,100},
    ytick={0.6, 0.7, 0.8, 0.9, 1.0},
    legend pos=south east,
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    ylabel style={yshift=-0.2cm},
    xlabel style={yshift=.17cm},
]
\addplot[
    color=blue,
    mark=o,
    mark size=2pt,
    ]
    coordinates {
    (1,	    0.6685745781)
    (5,	    0.7532774595)
    (10,	0.8110563812)
    (20,	0.8275062931)
    (30,	0.8435479993)
    (40,	0.8562941826)
    (50,	0.8609516933)
    (60,	0.8603157386)
    (70,	0.8625736454)
    (80,	0.8680444176)
    (90,	0.8794874775)
    (100,	0.8835495753)
    };
    \addlegendentry{Normal}
\addplot[
    color=red,
    mark=triangle,
    mark size=3pt,
    ]
    coordinates {
    (1,	    0.7659659027)
    (5,	    0.851032128)
    (10,	0.8633550726)
    (20,	0.8773286546)
    (30,	0.8829357742)
    (40,	0.8815846377)
    (50,	0.886550032)
    (60,	0.8837664467)
    (70,	0.8853310089)
    (80,	0.8886994934)
    (90,	0.8838568582)
    (100,	0.8846345938)
    };
    \addlegendentry{EDA}
\end{axis}
\end{tikzpicture}
\caption{Performance on text classification tasks with respect to percent of dataset used for training.}
\label{fig:single_saturation}
\end{centering}
\end{figure}

==> tables/individual_datasets.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{l||c|c|c|c|c|c}
\hline
 & \multicolumn{6}{c}{\textbf{Dataset}} \\ \hline
\textbf{Model} & SST2 & CR & SUBJ & TREC & PC & \textit{Average}\\ \hline \hline
RNN & 82.8 & 81.4 & 92.1 & 86.5 & 93.8 & 87.4 \\
\hspace{0.1cm}+EDA & 82.6 & 80.7 & 93.2 & 91.8 & 93.6 & 88.3 \\ \hline
CNN & 84.0 & 83.6 & 90.9 & 90.5 & 92.7 & 88.3 \\ 
\hspace{0.1cm}+EDA & 83.0 & 83.8 & 92.1 & 92.3 & 92.6 & 88.8 \\ \hline
\textit{Average} & 82.5 & 83.4 & 91.5 & 88.5 & 93.3 & 87.8 \\
\hspace{0.1cm}+EDA & 82.3 & 82.9 & 92.7 & 92.1 & 93.1 & 88.6 \\ \hline
\end{tabular}
\caption{Average performances (\%) across five text classification tasks on models trained with and without EDA. Training set sizes are $500$; $2$,$000$; $5$,$000$; and full data (all available data).}
\label{tab:individual_datasets}
\end{table*}
